Do you MIND? Reflections on the MIND dataset for research on diversity in news recommendations

The MIND dataset is at the moment of writing the most extensive dataset available for the research and development of news recommender systems. This work analyzes the suitability of the dataset for research on diverse news recommendations. On the one hand we analyze the effect the different steps in the recommendation pipeline have on the distribution of article categories, and on the other hand we check whether the supplied data would be sufficient for more sophisticated diversity analysis. We conclude that while MIND is a great step forward, there is still a lot of room for improvement.

==> 3_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\footnotesize
\caption{Distribution of the different article categories (the whole dataset, what was in the users' reading history, the dataset after candidate selection, and what the user clicked), and the recommender approaches. For the recommendations the top 8 items are selected. The distribution shown does not account for ranking.}
\label{tab:table_categories}
\begin{tabularx}{\linewidth}{l|YYYY|YY}
\textbf{}     & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{MIND}}                                                                    & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Recommendations}} \\ \cline{2-7} 
              & \cellcolor[HTML]{FFFFFF}all   & \cellcolor[HTML]{FFFFFF}candidate & \cellcolor[HTML]{FFFFFF}history & \cellcolor[HTML]{FFFFFF}clicked & \cellcolor[HTML]{FFFFFF}LSTUR     & \cellcolor[HTML]{FFFFFF}NRMS     \\ \hline
news          & \cellcolor[HTML]{F8696B}0,308 & \cellcolor[HTML]{FA8D72}0,234     & \cellcolor[HTML]{F9796E}0,277   & \cellcolor[HTML]{FA8C72}0,236   & \cellcolor[HTML]{FCA276}0,191     & \cellcolor[HTML]{FB9975}0,209    \\
sports        & \cellcolor[HTML]{F9786E}0,277 & \cellcolor[HTML]{FCB079}0,163     & \cellcolor[HTML]{FDB87B}0,145   & \cellcolor[HTML]{FA8771}0,246   & \cellcolor[HTML]{FA8971}0,243     & \cellcolor[HTML]{FA8C72}0,237    \\
finance       & \cellcolor[HTML]{FFE182}0,060 & \cellcolor[HTML]{FFDD82}0,068     & \cellcolor[HTML]{FFDD82}0,068   & \cellcolor[HTML]{DFE282}0,033   & \cellcolor[HTML]{E5E382}0,034     & \cellcolor[HTML]{CFDD81}0,031    \\
foodanddrink  & \cellcolor[HTML]{FFE583}0,053 & \cellcolor[HTML]{FFDE82}0,067     & \cellcolor[HTML]{FFE683}0,051   & \cellcolor[HTML]{FFE283}0,058   & \cellcolor[HTML]{FFD981}0,077     & \cellcolor[HTML]{FFDB81}0,074    \\
lifestyle     & \cellcolor[HTML]{FFE683}0,050 & \cellcolor[HTML]{FCAC78}0,171     & \cellcolor[HTML]{FECB7E}0,106   & \cellcolor[HTML]{FCA978}0,177   & \cellcolor[HTML]{FCB279}0,158     & \cellcolor[HTML]{FCA777}0,180    \\
travel        & \cellcolor[HTML]{FFE984}0,044 & \cellcolor[HTML]{B9D67F}0,027     & \cellcolor[HTML]{C9DB80}0,030   & \cellcolor[HTML]{91CB7D}0,020   & \cellcolor[HTML]{B1D47F}0,026     & \cellcolor[HTML]{BED880}0,028    \\
health        & \cellcolor[HTML]{FFEB84}0,040 & \cellcolor[HTML]{E4E382}0,034     & \cellcolor[HTML]{FFE884}0,046   & \cellcolor[HTML]{DFE182}0,033   & \cellcolor[HTML]{FFEA84}0,043     & \cellcolor[HTML]{FFEA84}0,043    \\
video         & \cellcolor[HTML]{F8E883}0,038 & \cellcolor[HTML]{93CC7D}0,020     & \cellcolor[HTML]{8AC97D}0,019   & \cellcolor[HTML]{9BCE7E}0,022   & \cellcolor[HTML]{99CD7E}0,021     & \cellcolor[HTML]{BFD880}0,028    \\
autos         & \cellcolor[HTML]{E8E482}0,035 & \cellcolor[HTML]{C9DB80}0,030     & \cellcolor[HTML]{EFE683}0,036   & \cellcolor[HTML]{AAD27F}0,024   & \cellcolor[HTML]{89C87D}0,018     & \cellcolor[HTML]{9BCE7E}0,022    \\
weather       & \cellcolor[HTML]{E5E382}0,034 & \cellcolor[HTML]{BDD880}0,028     & \cellcolor[HTML]{63BE7B}0,012   & \cellcolor[HTML]{72C27B}0,014   & \cellcolor[HTML]{A7D17E}0,024     & \cellcolor[HTML]{A5D17E}0,023    \\
tv            & \cellcolor[HTML]{8ECA7D}0,019 & \cellcolor[HTML]{FFE884}0,047     & \cellcolor[HTML]{FED780}0,082   & \cellcolor[HTML]{FFE784}0,049   & \cellcolor[HTML]{FFE383}0,056     & \cellcolor[HTML]{FFE984}0,043    \\
music         & \cellcolor[HTML]{73C27B}0,015 & \cellcolor[HTML]{FFE984}0,044     & \cellcolor[HTML]{BBD780}0,027   & \cellcolor[HTML]{E8E482}0,035   & \cellcolor[HTML]{FFE784}0,048     & \cellcolor[HTML]{FFEB84}0,040    \\
entertainment & \cellcolor[HTML]{6AC07B}0,013 & \cellcolor[HTML]{C4D980}0,029     & \cellcolor[HTML]{E6E382}0,035   & \cellcolor[HTML]{A4D07E}0,023   & \cellcolor[HTML]{FFEB84}0,039     & \cellcolor[HTML]{B4D57F}0,026    \\
movies        & \cellcolor[HTML]{67BF7B}0,013 & \cellcolor[HTML]{F8E983}0,038     & \cellcolor[HTML]{F6E883}0,037   & \cellcolor[HTML]{C7DA80}0,029   & \cellcolor[HTML]{92CB7D}0,020     & \cellcolor[HTML]{81C67C}0,017   
\end{tabularx}
\end{table}

==> archive.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\begin{tabular}{llllllllllllll}
 & news & sports & finance & \begin{tabular}[c]{@{}l@{}}foodand\\ drink\end{tabular} & lifestyle & travel & video & weather & autos & health & tv & music & \begin{tabular}[c]{@{}l@{}}entertain-\\ ment\end{tabular} \\
all & \cellcolor[HTML]{F8696B}0.303 & \cellcolor[HTML]{F96B6C}0.300 & \cellcolor[HTML]{FFE583}0.060 & \cellcolor[HTML]{FFEB84}0.048 & \cellcolor[HTML]{FFEB84}0.048 & \cellcolor[HTML]{FEEA83}0.047 & \cellcolor[HTML]{E6E382}0.041 & \cellcolor[HTML]{DCE182}0.039 & \cellcolor[HTML]{C8DB80}0.034 & \cellcolor[HTML]{C4DA80}0.033 & \cellcolor[HTML]{7AC47C}0.015 & \cellcolor[HTML]{70C17B}0.013 & \cellcolor[HTML]{65BE7B}0.010 \\
candidate & \cellcolor[HTML]{FA8A72}0.238 & \cellcolor[HTML]{FCA978}0.178 & \cellcolor[HTML]{FED17F}0.098 & \cellcolor[HTML]{FED580}0.091 & \cellcolor[HTML]{FCAA78}0.177 & \cellcolor[HTML]{FFE683}0.058 & \cellcolor[HTML]{FFE984}0.052 & \cellcolor[HTML]{FFEA84}0.050 & \cellcolor[HTML]{FFE683}0.059 & \cellcolor[HTML]{FFE283}0.066 & \cellcolor[HTML]{FFE082}0.071 & \cellcolor[HTML]{FFE583}0.060 & \cellcolor[HTML]{FFE984}0.051 \\
history & \cellcolor[HTML]{F9766E}0.279 & \cellcolor[HTML]{FDBB7B}0.142 & \cellcolor[HTML]{FFE082}0.069 & \cellcolor[HTML]{FFEA84}0.050 & \cellcolor[HTML]{FECE7F}0.105 & \cellcolor[HTML]{B7D67F}0.030 & \cellcolor[HTML]{89C97D}0.019 & \cellcolor[HTML]{6CC07B}0.012 & \cellcolor[HTML]{CFDD81}0.036 & \cellcolor[HTML]{FFEB84}0.047 & \cellcolor[HTML]{FFDA81}0.082 & \cellcolor[HTML]{ACD37F}0.027 & \cellcolor[HTML]{C9DB80}0.034 \\
lstur & \cellcolor[HTML]{FB9674}0.215 & \cellcolor[HTML]{FB9975}0.209 & \cellcolor[HTML]{FAE983}0.046 & \cellcolor[HTML]{FFDC82}0.078 & \cellcolor[HTML]{FCAB78}0.174 & \cellcolor[HTML]{9ECF7E}0.024 & \cellcolor[HTML]{92CB7D}0.021 & \cellcolor[HTML]{AFD47F}0.028 & \cellcolor[HTML]{8CCA7D}0.019 & \cellcolor[HTML]{FEEA83}0.047 & \cellcolor[HTML]{FAE983}0.046 & \cellcolor[HTML]{EAE582}0.042 & \cellcolor[HTML]{B2D57F}0.029 \\
pop & \cellcolor[HTML]{FCA878}0.179 & \cellcolor[HTML]{FDBF7C}0.135 & \cellcolor[HTML]{FFDB81}0.079 & \cellcolor[HTML]{FFE483}0.063 & \cellcolor[HTML]{FCA877}0.181 & \cellcolor[HTML]{D0DD81}0.036 & \cellcolor[HTML]{80C67C}0.016 & \cellcolor[HTML]{71C27B}0.013 & \cellcolor[HTML]{89C97D}0.019 & \cellcolor[HTML]{F5E883}0.045 & \cellcolor[HTML]{F3E783}0.044 & \cellcolor[HTML]{DDE182}0.039 & \cellcolor[HTML]{FFE082}0.070 \\
random & \cellcolor[HTML]{FA8F73}0.230 & \cellcolor[HTML]{FCB179}0.162 & \cellcolor[HTML]{FFE182}0.069 & \cellcolor[HTML]{FFE182}0.068 & \cellcolor[HTML]{FCAE79}0.169 & \cellcolor[HTML]{ABD37F}0.027 & \cellcolor[HTML]{90CB7D}0.020 & \cellcolor[HTML]{ADD37F}0.028 & \cellcolor[HTML]{B6D67F}0.030 & \cellcolor[HTML]{C9DB80}0.034 & \cellcolor[HTML]{FEEA83}0.047 & \cellcolor[HTML]{F1E783}0.044 & \cellcolor[HTML]{B3D57F}0.029
\end{tabular}
\caption{Distribution of the different article categories among the whole dataset, the dataset after candidate selection, what was in the users' reading history, and after the recommender approaches. For the recommender approaches the top 8 items are selected. The distribution shown does not account for ranking.}
\label{tab:table_categories}
\end{table*}

==> table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\setlength{\tabcolsep}{4pt}
%\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\textwidth}{X|XXXX|XXXX}{
>{\columncolor[HTML]{FFFFFF}}l |llll|llllll}
\textbf{}     & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{MIND Dataset}}                                                                     & \multicolumn{6}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Recommendations}}                                                                                                                                \\ \cline{2-11} 
              & \cellcolor[HTML]{FFFFFF}all    & \cellcolor[HTML]{FFFFFF}candidate & \cellcolor[HTML]{FFFFFF}history & \cellcolor[HTML]{FFFFFF}clicked & \cellcolor[HTML]{FFFFFF}lstur  & \cellcolor[HTML]{FFFFFF}npa    & \cellcolor[HTML]{FFFFFF}naml   & \cellcolor[HTML]{FFFFFF}nrms   & \cellcolor[HTML]{FFFFFF}pop    & \cellcolor[HTML]{FFFFFF}random \\ \cline{1-9}
news          & \cellcolor[HTML]{F8696B}0,3076 & \cellcolor[HTML]{FA8C72}0,2338    & \cellcolor[HTML]{F9786E}0,2765  & \cellcolor[HTML]{FA8C72}0,2357  & \cellcolor[HTML]{FBA176}0,1913 & \cellcolor[HTML]{FB9975}0,2077 & \cellcolor[HTML]{FB9E76}0,1973 & \cellcolor[HTML]{FB9875}0,2086 & \cellcolor[HTML]{FCA978}0,1737 & \cellcolor[HTML]{FA8D72}0,2328 \\
sports        & \cellcolor[HTML]{F9786E}0,2773 & \cellcolor[HTML]{FCAE79}0,1629    & \cellcolor[HTML]{FDB77A}0,1445  & \cellcolor[HTML]{FA8771}0,2462  & \cellcolor[HTML]{FA8871}0,2432 & \cellcolor[HTML]{FA8170}0,2578 & \cellcolor[HTML]{FA8671}0,2471 & \cellcolor[HTML]{FA8B72}0,2369 & \cellcolor[HTML]{FDBB7B}0,1367 & \cellcolor[HTML]{FCAE79}0,1635 \\
finance       & \cellcolor[HTML]{FFDF82}0,0604 & \cellcolor[HTML]{FFDB81}0,0684    & \cellcolor[HTML]{FFDB81}0,0684  & \cellcolor[HTML]{FFEB84}0,0335  & \cellcolor[HTML]{FFEB84}0,0345 & \cellcolor[HTML]{CFDD81}0,0234 & \cellcolor[HTML]{FFE984}0,0382 & \cellcolor[HTML]{F1E783}0,0306 & \cellcolor[HTML]{FFDC82}0,0656 & \cellcolor[HTML]{FFDB81}0,0685 \\
foodanddrink  & \cellcolor[HTML]{FFE283}0,0530 & \cellcolor[HTML]{FFDB81}0,0674    & \cellcolor[HTML]{FFE383}0,0507  & \cellcolor[HTML]{FFE082}0,0576  & \cellcolor[HTML]{FED781}0,0773 & \cellcolor[HTML]{FED680}0,0789 & \cellcolor[HTML]{FED781}0,0767 & \cellcolor[HTML]{FED881}0,0739 & \cellcolor[HTML]{FFE082}0,0582 & \cellcolor[HTML]{FFDB81}0,0677 \\
lifestyle     & \cellcolor[HTML]{FFE483}0,0502 & \cellcolor[HTML]{FCAA78}0,1711    & \cellcolor[HTML]{FEC97E}0,1057  & \cellcolor[HTML]{FCA777}0,1773  & \cellcolor[HTML]{FCB079}0,1584 & \cellcolor[HTML]{FCAF79}0,1603 & \cellcolor[HTML]{FCA877}0,1768 & \cellcolor[HTML]{FCA677}0,1804 & \cellcolor[HTML]{FCB27A}0,1538 & \cellcolor[HTML]{FCAA78}0,1709 \\
travel        & \cellcolor[HTML]{FFE784}0,0435 & \cellcolor[HTML]{DFE282}0,0268    & \cellcolor[HTML]{EDE582}0,0296  & \cellcolor[HTML]{BFD880}0,0199  & \cellcolor[HTML]{D9E081}0,0255 & \cellcolor[HTML]{EAE582}0,0291 & \cellcolor[HTML]{DDE182}0,0262 & \cellcolor[HTML]{E3E382}0,0276 & \cellcolor[HTML]{DDE182}0,0263 & \cellcolor[HTML]{E1E282}0,0272 \\
health        & \cellcolor[HTML]{FFE884}0,0404 & \cellcolor[HTML]{FFEB84}0,0342    & \cellcolor[HTML]{FFE583}0,0463  & \cellcolor[HTML]{FEEA83}0,0334  & \cellcolor[HTML]{FFE784}0,0429 & \cellcolor[HTML]{FFE583}0,0466 & \cellcolor[HTML]{FFE483}0,0485 & \cellcolor[HTML]{FFE784}0,0425 & \cellcolor[HTML]{FFE984}0,0387 & \cellcolor[HTML]{FFEB84}0,0345 \\
video         & \cellcolor[HTML]{FFE984}0,0377 & \cellcolor[HTML]{C1D980}0,0203    & \cellcolor[HTML]{BAD780}0,0187  & \cellcolor[HTML]{C8DB80}0,0217  & \cellcolor[HTML]{C6DA80}0,0213 & \cellcolor[HTML]{ABD27F}0,0156 & \cellcolor[HTML]{BED880}0,0196 & \cellcolor[HTML]{E5E382}0,0280 & \cellcolor[HTML]{F0E683}0,0303 & \cellcolor[HTML]{C1D980}0,0203 \\
autos         & \cellcolor[HTML]{FFEB84}0,0351 & \cellcolor[HTML]{EDE582}0,0297    & \cellcolor[HTML]{FFEA84}0,0362  & \cellcolor[HTML]{D3DE81}0,0242  & \cellcolor[HTML]{B8D67F}0,0184 & \cellcolor[HTML]{B9D67F}0,0186 & \cellcolor[HTML]{B4D57F}0,0174 & \cellcolor[HTML]{C8DB80}0,0217 & \cellcolor[HTML]{A2D07E}0,0135 & \cellcolor[HTML]{ECE582}0,0295 \\
weather       & \cellcolor[HTML]{FFEB84}0,0345 & \cellcolor[HTML]{E3E382}0,0275    & \cellcolor[HTML]{9ACD7E}0,0119  & \cellcolor[HTML]{A6D17E}0,0145  & \cellcolor[HTML]{D1DD81}0,0237 & \cellcolor[HTML]{EAE582}0,0291 & \cellcolor[HTML]{BCD780}0,0191 & \cellcolor[HTML]{CFDD81}0,0233 & \cellcolor[HTML]{EBE582}0,0293 & \cellcolor[HTML]{E4E382}0,0277 \\
tv            & \cellcolor[HTML]{BDD880}0,0194 & \cellcolor[HTML]{FFE583}0,0471    & \cellcolor[HTML]{FED480}0,0820  & \cellcolor[HTML]{FFE483}0,0485  & \cellcolor[HTML]{FFE182}0,0564 & \cellcolor[HTML]{FFE383}0,0503 & \cellcolor[HTML]{FFE383}0,0517 & \cellcolor[HTML]{FFE784}0,0435 & \cellcolor[HTML]{DBE081}0,0259 & \cellcolor[HTML]{FFE583}0,0473 \\
music         & \cellcolor[HTML]{A7D17E}0,0147 & \cellcolor[HTML]{FFE684}0,0443    & \cellcolor[HTML]{E1E282}0,0271  & \cellcolor[HTML]{FFEB84}0,0350  & \cellcolor[HTML]{FFE583}0,0478 & \cellcolor[HTML]{FFEA84}0,0370 & \cellcolor[HTML]{F4E783}0,0311 & \cellcolor[HTML]{FFE884}0,0399 & \cellcolor[HTML]{FED480}0,0839 & \cellcolor[HTML]{FFE684}0,0441 \\
entertainment & \cellcolor[HTML]{A0CF7E}0,0132 & \cellcolor[HTML]{E8E482}0,0287    & \cellcolor[HTML]{FFEB84}0,0346  & \cellcolor[HTML]{CFDD81}0,0233  & \cellcolor[HTML]{FFE984}0,0391 & \cellcolor[HTML]{F2E783}0,0309 & \cellcolor[HTML]{FFEA84}0,0359 & \cellcolor[HTML]{DBE081}0,0259 & \cellcolor[HTML]{FFD981}0,0725 & \cellcolor[HTML]{E6E382}0,0281 \\
movies        & \cellcolor[HTML]{9ECF7E}0,0127 & \cellcolor[HTML]{FFE984}0,0378    & \cellcolor[HTML]{FFEA84}0,0374  & \cellcolor[HTML]{EBE582}0,0292  & \cellcolor[HTML]{C0D980}0,0201 & \cellcolor[HTML]{A7D17E}0,0147 & \cellcolor[HTML]{A5D17E}0,0142 & \cellcolor[HTML]{B2D57F}0,0172 & \cellcolor[HTML]{FED07F}0,0916 & \cellcolor[HTML]{FFE984}0,0380
\end{tabularx}
